Exponential Separation of Quantum and Classical One-Way Numbers-on-Forehead Communication

Numbers-on-Forehead (NOF) communication model is a central model in communication complexity. As a restricted variant, one-way NOF model is of particular interest. Establishing strong one-way NOF lower bounds would imply circuit lower bounds, resolve well-known problems in additive combinatorics, and yield wide-ranging applications in areas such as cryptography and distributed computing. However, proving strong lower bounds in one-way NOF communication remains highly challenging; many fundamental questions in one-way NOF communication remain wide open. One of the fundamental questions, proposed by Gavinsky and Pudl\'ak (CCC 2008), is to establish an explicit exponential separation between quantum and classical one-way NOF communication. In this paper, we resolve this open problem by establishing the first exponential separation between quantum and randomized communication complexity in one-way NOF model. Specifically, we define a lifted variant of the Hidden Matching problem of Bar-Yossef, Jayram, and Kerenidis (STOC 2004) and show that it admits an ($O(\log n)$)-cost quantum protocol in the one-way NOF setting. By contrast, we prove that any $k$-party one-way randomized protocol for this problem requires communication $\Omega(\frac{n^{1/3}}{2^{k/3}})$. Notably, our separation applies even to a generalization of $k$-player one-way communication, where the first player speaks once, and all other $k-1$ players can communicate freely.

==> Discussion.tex <==
\section{Discussion and Open Problems}
A natural open problem is to extend our lifting theorem to the randomized setting. Specifically, we propose the following conjecture:

\begin{conjecture}\label{main_conjecture}
For any partial function $f : [q] \times [q] \to \{0,1\}$, we have
\[
\mathrm{ORCC^{NOF}}(f \circ \gip) = \Theta(\mathrm{ORCC}(f)),
\]
where $\mathrm{ORCC}(f)$ denotes the one-way randomized communication complexity of $f$, and $\mathrm{ORCC^{NOF}}(f \circ \gip)$ denotes the one-way number-on-forehead (NOF) randomized communication complexity of $f \circ \gip$.
\end{conjecture}

Proving this conjecture would imply a separation between quantum and classical communication complexity in the one-way NOF model.

Another important open problem is to extend our lifting theorem (Theorem~\ref{main_theorem}) to general communication protocols beyond the one-way setting. Such a result could provide an optimal separation between randomized and deterministic NOF communication.

==> RCCLifting.tex <==
\section{Lifting Theorems for One-Way NOF Communication}

\subsection{Deterministic vs Randomized in NOF}
\paragraph{Related Works:}
\begin{enumerate}
    \item $\Omega(\sqrt{n})$ vs $O(1)$ for $\textbf{EQ}(\textbf{IP}(x_3,x_2),\textbf{IP}(x_3,x_1),\textbf{IP}(x_1,x_2))$ in general NOF model \cite{kelley2024explicit,kelley2025efficientsiftinggridnorms}.
    \item $\Omega(\frac{n}{2^k})$ vs $O(1)$ for $\textbf{EQ}(x_k,\textbf{IP}(x_1,...,x_{k-1}))$ in one-way NOF model \cite{yang2025deterministic}.
\end{enumerate}

\begin{conjecture}\label{Conjecture}
There exist constants $k,\varepsilon>0$ and an explicit function $f : [N]\times [N] \to [q]$, where $N = q^k$, such that for every sufficiently large $q$ and every subset $S \subseteq [N]\times [N]$ with $|S| \ge \frac{N^2}{q^\varepsilon}$, there exist $y,z,y',z' \in [N]$ such that
\[
(y,z),\ (y',z),\ (y,z') \in S \quad \text{and} \quad f(y,z) \neq f(y',z) = f(y,z').
\]
\end{conjecture}

\begin{theorem}
For $F(x,y,z) = EQ(x,f(y,z))$, if Conjecture \ref{Conjecture} holds, then $\log \chi(F) = \Omega(\log N)$.
\end{theorem}

\begin{proof}
Let $\chi(F)$ be the minimum number of $1$-monochromatic cylinder intersections needed to cover the $1$-inputs of $F$. Let $\mathcal{C}$ be such a covering. For each $C \in \mathcal{C}$, define its projection onto the $(y,z)$ coordinates:
\[
S_C := \{ (y,z) \in [N]^2 \mid \exists x \in [q], (x,y,z) \in C \}.
\]
Since each $(y,z)$ corresponds to exactly one $x = f(y,z)$ such that $F(x,y,z)=1$, the sets $\{S_C\}_{C \in \mathcal{C}}$ form a partition of $[N]^2$. By the pigeonhole principle, there exists a $C \in \mathcal{C}$ such that:
\[
|S_C| \ge \frac{N^2}{\chi(F)}.
\]

Suppose for contradiction that $\chi(F) \le q^\varepsilon$. Then $|S_C| \ge N^2/q^\varepsilon$. By Conjecture \ref{Conjecture}, there exist $(y,z), (y',z), (y,z') \in S_C$ such that:
\[
f(y,z) \neq f(y',z) = f(y,z') = a.
\]
By the definition of $S_C$ and the fact that $C$ is $1$-monochromatic, the triples $(a, y', z)$ and $(a, y, z')$ must both be in $C$. 

Since $(y,z)\in S_C$, there is a $a'\in [q]$ such that $(a',y,z)\in C$. Thus, by $(a, y', z) \in C$ and $(a, y, z') \in C$ and $(a',y,z)\in C$ and the cylinder intersection property, implies that
\[
(a, y, z) \in C.
\]
Because $C$ is a $1$-monochromatic cylinder intersection for $F$, every element in $C$ must satisfy $x = f(y,z)$. This implies $a = f(y,z)$, which contradicts our earlier condition that $f(y,z) \neq a$.

Consequently, we must have $\chi(F) > q^\varepsilon$. Taking logarithms:
\[
\log \chi(F) > \varepsilon \log q = \frac{\varepsilon}{k} \log N.
\]
Thus, $\log \chi(F) = \Omega(\log N)$.
\end{proof}

\subsection{Size-Depth Trade-off of Boolean Circuits}


==> macros.tex <==

%shaded theorem environments
\newtheorem{theorem}{Theorem}[section]
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{definition}

\newtheorem{definition}[theorem]{Definition}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{example}[theorem]{Example}
\newtheorem{protocol}[theorem]{Protocol}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{remark}[theorem]{Remark}


\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\size}[1]{\left| #1 \right|}
\newcommand{\cond}[2]{\left. #1 \right|_{#2}}

\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\tuple}[1]{\left(#1\right)} \newcommand{\eps}{\varepsilon}
\newcommand{\inner}[2]{\langle #1,#2\rangle} \newcommand{\tp}{\tuple}
\renewcommand{\mid}{\;\middle\vert\;} \newcommand{\cmid}{\,:\,}
\newcommand{\numP}{\#\mathbf{P}} \renewcommand{\P}{\mathbf{P}}
\newcommand{\defeq}{\triangleq} \renewcommand{\d}{\,\-d}
\newcommand{\ol}{\overline}
\newcommand{\wt}{\widetilde}
\newcommand{\wh}{\widehat}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\eqdef}{\stackrel{\mathsf{def}}{=}}
\newcommand{\bool}{\set{-1 , 1}^n \to \set{-1, 1}}
\newcommand{\rv}[1]{\boldsymbol{#1}}
\newcommand{\zo}{\set{0,1}}

\newcommand{\N}{\mathbb{N}}
\newcommand{\ee}{\mathcal{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\dd}{\mathcal{D}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\gFam}{\mathcal{G}}
\newcommand{\fFam}{\mathcal{F}}
\newcommand{\hFam}{\mathcal{H}}
\renewcommand{\aa}{\mathcal{A}}
\newcommand{\bb}{\mathcal{B}}
\newcommand{\ii}{\mathcal{I}}
\newcommand{\rr}{\mathcal{R}}
\newcommand{\qq}{\mathcal{Q}}
\newcommand{\xx}{\mathcal{X}}
\newcommand{\mm}{\mathcal{M}}
\newcommand{\yy}{\mathcal{Y}}
\renewcommand{\ss}{\mathcal{S}}
\renewcommand{\ll}{\mathcal{L}}
\renewcommand{\tt}{\mathcal{T}}
\newcommand{\view}{\mathcal{V}}

\newcommand{\alice}{\mathsf{A}}
\newcommand{\bob}{\mathsf{B}}
\newcommand{\charlie}{\mathsf{C}}
\newcommand{\eve}{\mathsf{E}}
\newcommand{\party}{\mathsf{P}}

\newcommand{\OCC}{\mathrm{OCC}}

\newcommand{\supp}{\mathrm{supp}}
\newcommand{\KL}[2]{\mathrm{KL}\left(#1\middle\|#2\right)}
\newcommand{\SD}[2]{\mathsf{SD}\left(#1 ; #2\right)}
\newcommand{\msf}{\mathsf}
\newcommand{\mbf}{\mathbf}
\newcommand{\true}{\textsc{True}}
\newcommand{\false}{\textsc{False}}
\newcommand{\s}{\mathcal{S}}
\newcommand{\CF}{\mathsf{CF}}
\newcommand{\reduction}{\mathsf{R}}
\newcommand{\adv}{\mathtt{Adv}}
\newcommand{\expt}{\mathsf{Expt}}
\newcommand{\D}{\mathtt{D}}
\newcommand{\range}{\mathrm{range}}
\newcommand{\EQUAL}{\mathrm{EQ}}
\newcommand{\IP}{\mathrm{IP}}
\newcommand{\GGIP}{\mathrm{GIP}}

%\renewcommand{\thealgorithm}{} %% disable the algorithm counter

\newcommand{\stress}[1]{\textcolor{black}{\textbf{\textit{#1}}}}
\renewcommand{\emph}[1]{\textbf{\textit{#1}}}

\renewcommand{\Pr}{\operatorname*{\mathbf{Pr}}}
\DeclareMathOperator*{\E}{\mathbf{E}}
\DeclareMathOperator*{\ent}{\mathbf{H}}
\DeclareMathOperator*{\minent}{\mathbf{H}_{\infty}}
\DeclareMathOperator*{\maxent}{\mathbf{H}_{\msf{max}}}
\newcommand{\I}{\mathrm{I}}
\newcommand{\mutual}[2]{\mathrm{I}\left(#1; #2\right)}
\newcommand{\condmutual}[3]{\mathrm{I}\left(#1; #2 \mid #3\right)}

\newcommand{\sd}{\mathtt{SD}}
\newcommand{\pr}[2][]{ \ifthenelse{\isempty{#1}}
  {\Pr\left[#2\right]} {\Pr_{#1}\left[#2\right]} }
\newcommand{\ex}[2][]{ \ifthenelse{\isempty{#1}}
  {\E\left[#2\right]}
  {\E_{#1}\left[#2\right]} }

\newcommand{\algo}[1]{\mathsf{#1}}
\newcommand{\poly}{\mathtt{poly}}
\newcommand{\negl}{\mathtt{negl}}

%complexity classes
\newcommand{\polytime}{\mathbf{P}}
\newcommand{\NP}{\mathbf{NP}}
\newcommand{\EXP}{\mathsf{EXP}}
\newcommand{\PCP}{\mathbf{PCP}}
\newcommand{\DTIME}{\mathbf{DTIME}}
\newcommand{\NTIME}{\mathbf{NTIME}}
\newcommand{\PPT}{\textsc{ PPT }}
\newcommand{\CC}{\mathrm{CC}}

\newcommand{\hamming}{\mathtt{HW}}
\newcommand{\hammingd}{\mathtt{HD}}
\newcommand{\rhammingd}{\mathtt{rHD}}
\newcommand{\val}{\mathtt{val}}
\newcommand{\Img}{\mathtt{Im}}
\newcommand{\dom}{\mathtt{Dom}}

\newcommand{\resp}{resp.,\ }
\newcommand{\ie} {i.e.,\ }
\newcommand{\eg} {e.g.,\ }
%\newcommand{\GHM}{\text{HM}}

\crefname{algocf}{alg.}{algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\newcommand{\restrict}[1]{(#1)}
